Listening to Patients: A Framework of Detecting and Mitigating Patient Misreport for Medical Dialogue Generation

Medical Dialogue Systems aim to provide automated healthcare support through patient-agent conversations. Previous efforts typically regard patients as ideal users -- one who accurately and consistently reports their health conditions. However, in reality, patients often misreport their symptoms, leading to discrepancies between their reports and actual health conditions. Overlooking patient misreport will affect the quality of healthcare consultations provided by MDS. To address this issue, we argue that MDS should ''listen to patients'' and tackle two key challenges: how to detect and mitigate patient misreport effectively. In this work, we propose PaMis, a framework of detecting and mitigating Patient Misreport for medical dialogue generation. PaMis first constructs dialogue entity graphs, then detects patient misreport based on graph entropy, and mitigates patient misreport by formulating clarifying questions. Experiments indicate that PaMis effectively enhances medical response generation, enabling models like GPT-4 to detect and mitigate patient misreports, and provide high-quality healthcare assistance.

==> tables/llms_winrate.tex <==

% LLMs win rate
\begin{table}[t]
\tiny
    \centering
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule[1.2pt]
        \textbf{ V.S.}
        & \textbf{ ChatGPT }
        & \textbf{ RAG (plain) }
        & \textbf{ RAG (weighted) }
        \\
        \midrule[0.8pt]
        \textbf{ P } &+ 27.59\% &+ 13.79\% &+ 8.19\% \\
        \textbf{ A } &+ 28.02\% &+ 12.07\% &+ 5.17\% \\
        \textbf{ H } &+ 28.88\% &+ 23.28\% &+ 8.62\% \\
        \textbf{ LQ } &+ 16.38\% &+ 9.48\% &+ 6.03\% \\
        \textbf{ DV } &+ 28.45\% &+ 13.36\% &+ 6.90\%  \\
        \midrule[0.8pt]
        \midrule[0.8pt]
        \textbf{ V.S.}
        & \textbf{ GPT-4 }
        & \textbf{ RAG (plain) }
        & \textbf{ RAG (weighted) }
        \\
        \midrule[0.8pt]
        \textbf{ P } &+ 0.87\% &+ 14.85\% &+ 9.17\% \\
        \textbf{ A } &+ 3.49\% &+ 3.06\% &- 0.87\% \\
        \textbf{ H } &+ 3.06\% &+ 10.04\% &+ 0.44\% \\
        \textbf{ LQ } &- 1.31\% &+ 4.80\% &+ 1.75\% \\
        \textbf{ DV } &+ 10.92\% &+ 15.72\% &+ 19.21\% \\
        \bottomrule[1.2pt]
    \end{tabular}}
    \caption{The difference in win rate between \modelname{} and baseline methods.}
    \label{tab:llms_winrate}

\end{table}
